Quantifying the Privacy Risks of Learning High-Dimensional Graphical Models

Models leak information about their training data. This enables attackers to infer sensitive information about their training sets, notably determine if a data sample was part of the model's training set. The existing works empirically show the possibility of these membership inference (tracing) attacks against complex deep learning models. However, the attack results are dependent on the specific training data, can be obtained only after the tedious process of training the model and performing the attack, and are missing any measure of the confidence and unused potential power of the attack. In this paper, we theoretically analyze the maximum power of tracing attacks against high-dimensional graphical models, with the focus on Bayesian networks. We provide a tight upper bound on the power (true positive rate) of these attacks, with respect to their error (false positive rate), for a given model structure even before learning its parameters. As it should be, the bound is independent of the knowledge and algorithm of any specific attack. It can help in identifying which model structures leak more information, how adding new parameters to the model increases its privacy risk, and what can be gained by adding new data points to decrease the overall information leakage. It provides a measure of the potential leakage of a model given its structure, as a function of the model complexity and the size of the training set.

==> sections/Assumptions.tex <==
% !TEX root = ../main.tex
\section{Theoretical analysis}\label{sec:assumptions}

%\textit{Assumptions:} 
To derive our main result about the best achievable power-error tradeoff, we assume that the released parameters satisfy the below conditions.

\begin{itemize}
	\item The value of every released parameter is learned from a large enough number of samples for the central limit theorem to hold good. 
	\item The value of every released parameter is non-trivial i.e., it is bounded away from 0 and 1~\cite{sankararaman2009genomic}.
\end{itemize}

These are valid assumptions to make on part of the model publisher, as it is not beneficial to publish statistically insignificant or trivial estimates. In fact, the recently published methodology of learning Bayesian Networks on Cancer Analysis System (CAS) database in the National Cancer Registration and Analysis Service (NCRAS) has similar assumptions (they use only the parameters that are learned using at least 50 samples)~\cite{Simulacrum}. 

==> sections/figure_estimationerror.tex <==
% !TEX root = ../main.tex
\begin{figure}
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tikzpicture}


\begin{axis}[
xmin=-4.5,xmax=4.5,
ymin=0,ymax=0.5,
xtick={ -0.8, 0,  1.72},
xticklabels={$\mu_{D'}$, $\mu$, $\mu_D$},
axis on top,
legend style={legend cell align=right,legend plot pos=right}] 
\addplot[color=red,domain=-5:5,samples=100] {1/sqrt(2*pi)*exp(-x^2/2)};
\addplot[dashed, color=blue,domain=-5:5,samples=100] {1/sqrt(8*pi)*exp(-x^2/8)};


\draw[red,thick] (-0.8,0) -- (-0.8, 0.29);
\draw[red,thick] (1.72,0) -- (1.72, 0.14);

\addlegendentry{$\theta \sim \mathcal{N}(\mu, \sigma^2)$}
\addlegendentry{$\theta \sim \mathcal{N}(\mu, 2\sigma^2 )$}

\filldraw[red] (-0.8, 0.29) circle (2pt)  ;
\filldraw[blue] (1.72, 0.14) circle (2pt) ;
\filldraw[blue] (-0.8, 0.185) circle (2pt)  ;
\filldraw[red] (1.72, 0.09) circle (2pt) ;

\node at (axis cs:2.175,0.14) {$D$};
\node at (axis cs:-0.34,0.29) {$D'$};

\end{axis}
\end{tikzpicture}
}	
\caption{\small{Distribution of the statistic $\theta$ (mean) estimated over different datasets of size $n$ (and $\frac{n}{2}$) sampled iid from $P$. The dashed line corresponds to the datasets of size $\frac{n}{2}$. The mean of $P$ is denoted by $\mu$. The larger the deviation of $\mu_D$ from $\mu$ is, the easier it is to distinguish dataset $D$ from other datasets of equal size. The smaller the size of $D$ is, the easier it is to distinguish dataset $D$ from other datasets of equal size. {}}}
 
 \vspace{-1.5em}
\label{fig:meanDistri}
\end{figure}




